Topic-switch adapted Japanese Dialogue System based on PLATO-2

Large-scale open-domain dialogue systems such as PLATO-2 have achieved state-of-the-art scores in both English and Chinese. However, little work explores whether such dialogue systems also work well in the Japanese language. In this work, we create a large-scale Japanese dialogue dataset, Dialogue-Graph, which contains 1.656 million dialogue data in a tree structure from News, TV subtitles, and Wikipedia corpus. Then, we train PLATO-2 using Dialogue-Graph to build a large-scale Japanese dialogue system, PLATO-JDS. In addition, to improve the PLATO-JDS in the topic switch issue, we introduce a topic-switch algorithm composed of a topic discriminator to switch to a new topic when user input differs from the previous topic. We evaluate the user experience by using our model with respect to four metrics, namely, coherence, informativeness, engagingness, and humanness. As a result, our proposed PLATO-JDS achieves an average score of 1.500 for the human evaluation with human-bot chat strategy, which is close to the maximum score of 2.000 and suggests the high-quality dialogue generation capability of PLATO-2 in Japanese. Furthermore, our proposed topic-switch algorithm achieves an average score of 1.767 and outperforms PLATO-JDS by 0.267, indicating its effectiveness in improving the user experience of our system.

==> JSAI 2023/data_en.tex <==
\usepackage{color}
	
%%Title: 
\title{How to use the \LaTeX{} Style File for English Manuscripts for JSAI20XX}

%%Contact address: 
\address{Name, Affiliation, Address, Phone number, Facsimile number, and E-mail address}

%%Name of authors:
\author{%
The Program Committee of the JSAI20XX\first
\and
Second Author's Name\second
}

%%Affiliations:
\affiliate{
\first{} The Japanese Society for Artificial Intelligence
\and
\second{} Affiliation \#2
}

%%
%\Vol{28}        %% <-- 25
%\session{0A0-00}%% <-- ID

\begin{abstract}
Here is an abstract of up to 150 words in English. 
This document describes the formatting guidelines for English manuscripts in \LaTeX{} of the annual conference of JSAI. This is also a sample of a formatted manuscript (see 2.4 for writing the abstract).
\end{abstract}

%\setcounter{page}{1}
\def\Style{``jsaiac.sty''}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em%
 T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\JBibTeX{\leavevmode\lower .6ex\hbox{J}\kern-0.15em\BibTeX}
\def\LaTeXe{\LaTeX\kern.15em2$_{\textstyle\varepsilon}$}

\begin{document}
\maketitle

\section{Introduction}

This article contains format guidelines for authors contributing to JSAI 20XX using \LaTeX{}. The conference proceedings will be distributed on a conference Web site containing PDF files prepared by the authors. To ensure that all papers in the proceedings have a uniform appearance, please refer to the following instructions. \textcolor{red}{This information may be updated even after it is released. Please confirm that it is the latest version before your submission.}


\section{General Information}
\subsection{File format and size}

The manuscript file should be an Adobe(R) PDF (Portable Document Format) file. The size of the manuscript file should be less than 3 Mbytes. The extension of the file name should be ``.pdf".

\subsection{Header}

The conference name in the header and your paper ID should not be included, because the organizing committee will add them.

\subsection{Title and author's name(s)}

The title of the paper and author's name(s) should be the same as those appeared in the application form. \textcolor{red}{Please ensure there are no differences between title and author's name(s) in the manuscript and presentation application.}

\subsection{Abstract}

Please include (1) the objective and (2) the outline of the conclusions of your results in the abstract under the author information. Also, please state the outline of your method as necessary in the abstract.  \textcolor{red}{Submissions without any description regarding (1) or (2) in the abstract may not be considered for presentation or publication.}

\subsection{Paper length}

The length of each paper is two pages on A4 size paper. Up to two additional pages are accepted.

\subsection{International session}

English is the only acceptable language for the international sessions. Papers for the international sessions will be included on the conference Web site, from which selected papers will be included in the post-proceedings after substantial extension.

\section{Style file for \LaTeX{}}

When you use the style file for JSAI20XX named ``jsaiac.sty'', please specify a style option as follows;

For \LaTeX{}2.09, 
\begin{verbatim}
\documentstyle[twocolumn,jsaiac]{article}
\end{verbatim}

For \LaTeXe{}, 
\begin{verbatim}
\documentclass[twocolumn]{article}
\usepackage{jsaiac}
\end{verbatim}


\def\Label{\vskip.5\baselineskip\noindent$\circ$\hskip3pt{}}

\Label The first page: 
Please use the following commands;
\begin{itemize}
\item Title: 
\begin{verbatim}
\title{Title of your paper}
\end{verbatim}

\item Name of authors:
\begin{verbatim}
\author{%
   Name of the first author\first{}
\and
   Name of the second author\second{}
}
\end{verbatim}

If the affiliations of authors are different, please use the following commands;

\begin{verbatim}
\def\first{\hbox{$\m@th^{\ast 1}$\hss}}
\def\second{\hbox{$\m@th^{\ast 2}$\hss}}
\def\third{\hbox{$\m@th^{\ast 3}$\hss}}
\def\fourth{\hbox{$\m@th^{\ast 4}$\hss}}
\def\fifth{\hbox{$\m@th^{\ast 5}$\hss}}
\def\sixth{\hbox{$\m@th^{\ast 6}$\hss}}
\def\seventh{\hbox{$\m@th^{\ast 7}$\hss}}
\def\eighth{\hbox{$\m@th^{\ast 8}$\hss}}
\def\ninth{\hbox{$\m@th^{\ast 9}$\hss}}
\end{verbatim}

You should add the same commands for corresponding affiliations. 
If there is only one affiliation, the \verb|\first| is not needed.

\item Affiliations: 
\begin{verbatim}
\affiliate{
   \first{}Affiliation #1
\and
   \second{}Affiliation #2
\and
   \third{}Affiliation #3
}
\end{verbatim}

\item Contact address: 
Use the \verb|\address| command as follows;

\begin{verbatim}
\address{name, affiliation, address, 
phone number, Fax number, 
e-mail address}
\end{verbatim}
\end{itemize}

\Label Misc.
\begin{itemize}
\item References: The style of the Journal of JSAI is preferred.
Some samples are shown below.

\end{itemize}

\begin{thebibliography}{99}
\bibitem[Knuth 84]{texbook}
 Knuth,~D.~E.: The \TeX{}book, Addison-Wesley (1984),
\bibitem[Lamport 86]{latexbook}
Leslie,~L: \LaTeX{}: {A} Document Preparation System (Updated for
  \LaTeX{}2$\varepsilon$), Addison-Wesley, 2nd edition (1998)
\end{thebibliography}
%%













==> data_en.tex <==
\usepackage{color}
	
%%Title: 
\title{How to use the \LaTeX{} Style File for English Manuscripts for JSAI20XX}

%%Contact address: 
\address{Name, Affiliation, Address, Phone number, Facsimile number, and E-mail address}

%%Name of authors:
\author{%
The Program Committee of the JSAI20XX\first
\and
Second Author's Name\second
}

%%Affiliations:
\affiliate{
\first{} The Japanese Society for Artificial Intelligence
\and
\second{} Affiliation \#2
}

%%
%\Vol{28}        %% <-- 25
%\session{0A0-00}%% <-- ID

\begin{abstract}
Here is an abstract of up to 150 words in English. 
This document describes the formatting guidelines for English manuscripts in \LaTeX{} of the annual conference of JSAI. This is also a sample of a formatted manuscript (see 2.4 for writing the abstract).
\end{abstract}

%\setcounter{page}{1}
\def\Style{``jsaiac.sty''}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em%
 T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
\def\JBibTeX{\leavevmode\lower .6ex\hbox{J}\kern-0.15em\BibTeX}
\def\LaTeXe{\LaTeX\kern.15em2$_{\textstyle\varepsilon}$}

\begin{document}
\maketitle

\section{Introduction}

This article contains format guidelines for authors contributing to JSAI 20XX using \LaTeX{}. The conference proceedings will be distributed on a conference Web site containing PDF files prepared by the authors. To ensure that all papers in the proceedings have a uniform appearance, please refer to the following instructions. \textcolor{red}{This information may be updated even after it is released. Please confirm that it is the latest version before your submission.}


\section{General Information}
\subsection{File format and size}

The manuscript file should be an Adobe(R) PDF (Portable Document Format) file. The size of the manuscript file should be less than 3 Mbytes. The extension of the file name should be ``.pdf".

\subsection{Header}

The conference name in the header and your paper ID should not be included, because the organizing committee will add them.

\subsection{Title and author's name(s)}

The title of the paper and author's name(s) should be the same as those appeared in the application form. \textcolor{red}{Please ensure there are no differences between title and author's name(s) in the manuscript and presentation application.}

\subsection{Abstract}

Please include (1) the objective and (2) the outline of the conclusions of your results in the abstract under the author information. Also, please state the outline of your method as necessary in the abstract.  \textcolor{red}{Submissions without any description regarding (1) or (2) in the abstract may not be considered for presentation or publication.}

\subsection{Paper length}

The length of each paper is two pages on A4 size paper. Up to two additional pages are accepted.

\subsection{International session}

English is the only acceptable language for the international sessions. Papers for the international sessions will be included on the conference Web site, from which selected papers will be included in the post-proceedings after substantial extension.

\section{Style file for \LaTeX{}}

When you use the style file for JSAI20XX named ``jsaiac.sty'', please specify a style option as follows;

For \LaTeX{}2.09, 
\begin{verbatim}
\documentstyle[twocolumn,jsaiac]{article}
\end{verbatim}

For \LaTeXe{}, 
\begin{verbatim}
\documentclass[twocolumn]{article}
\usepackage{jsaiac}
\end{verbatim}


\def\Label{\vskip.5\baselineskip\noindent$\circ$\hskip3pt{}}

\Label The first page: 
Please use the following commands;
\begin{itemize}
\item Title: 
\begin{verbatim}
\title{Title of your paper}
\end{verbatim}

\item Name of authors:
\begin{verbatim}
\author{%
   Name of the first author\first{}
\and
   Name of the second author\second{}
}
\end{verbatim}

If the affiliations of authors are different, please use the following commands;

\begin{verbatim}
\def\first{\hbox{$\m@th^{\ast 1}$\hss}}
\def\second{\hbox{$\m@th^{\ast 2}$\hss}}
\def\third{\hbox{$\m@th^{\ast 3}$\hss}}
\def\fourth{\hbox{$\m@th^{\ast 4}$\hss}}
\def\fifth{\hbox{$\m@th^{\ast 5}$\hss}}
\def\sixth{\hbox{$\m@th^{\ast 6}$\hss}}
\def\seventh{\hbox{$\m@th^{\ast 7}$\hss}}
\def\eighth{\hbox{$\m@th^{\ast 8}$\hss}}
\def\ninth{\hbox{$\m@th^{\ast 9}$\hss}}
\end{verbatim}

You should add the same commands for corresponding affiliations. 
If there is only one affiliation, the \verb|\first| is not needed.

\item Affiliations: 
\begin{verbatim}
\affiliate{
   \first{}Affiliation #1
\and
   \second{}Affiliation #2
\and
   \third{}Affiliation #3
}
\end{verbatim}

\item Contact address: 
Use the \verb|\address| command as follows;

\begin{verbatim}
\address{name, affiliation, address, 
phone number, Fax number, 
e-mail address}
\end{verbatim}
\end{itemize}

\Label Misc.
\begin{itemize}
\item References: The style of the Journal of JSAI is preferred.
Some samples are shown below.

\end{itemize}

\begin{thebibliography}{99}
\bibitem[Knuth 84]{texbook}
 Knuth,~D.~E.: The \TeX{}book, Addison-Wesley (1984),
\bibitem[Lamport 86]{latexbook}
Leslie,~L: \LaTeX{}: {A} Document Preparation System (Updated for
  \LaTeX{}2$\varepsilon$), Addison-Wesley, 2nd edition (1998)
\end{thebibliography}
%%












